Extended MSO Model Checking via Small Vertex Integrity

We study the model checking problem of an extended $\mathsf{MSO}$ with local and global cardinality constraints, called $\mathsf{MSO}^{\mathsf{GL}}_{\mathsf{Lin}}$, introduced recently by Knop, Kouteck\'{y}, Masa\v{r}\'{i}k, and Toufar [Log. Methods Comput. Sci., 15(4), 2019]. We show that the problem is fixed-parameter tractable parameterized by vertex integrity, where vertex integrity is a graph parameter standing between vertex cover number and treedepth. Our result thus narrows the gap between the fixed-parameter tractability parameterized by vertex cover number and the W[1]-hardness parameterized by treedepth.

==> fix-bibunits-hyperref.tex <==
\makeatletter
\def\hyper@natlinkstart#1{%
  \Hy@backout{#1}%
  \hyper@linkstart{cite}{cite.\@bibunitname.#1}%
%                             ^^^^^^^^^^^^^^
  \def\hyper@nat@current{#1}%
}

\def\hyper@natlinkbreak#1#2{%
  \hyper@linkend#1\hyper@linkstart{cite}{cite.\@bibunitname.#2}%
%                                             ^^^^^^^^^^^^^^
}

\def\hyper@natanchorstart#1{%
  \hyper@anchorstart{cite.\@bibunitname.#1}%
%                         ^^^^^^^^^^^^^^
}

\def\bibcite#1#2{%
  \@newl@bel{b}{#1}{\hyper@@link[cite]{}{cite.\@bibunitname.#1}{#2}}%
%                                             ^^^^^^^^^^^^^^
}%

\def\@lbibitem[#1]#2{%
  \@skiphyperreftrue
  \H@item[\hyper@anchorstart{cite.\@bibunitname.#2}%
%                                 ^^^^^^^^^^^^^^
  \@BIBLABEL{#1}\hyper@anchorend\hfill]%
  \@skiphyperreffalse
  \if@filesw
    \begingroup
      \let\protect\noexpand
      \immediate\write\@auxout{%
        \string\bibcite{#2}{#1}%
      }%
    \endgroup
  \fi
  \ignorespaces
}%

\def\@bibitem#1{%
  \@skiphyperreftrue\H@item\@skiphyperreffalse
  \hyper@anchorstart{cite.\@bibunitname.#1}\relax\hyper@anchorend
%                         ^^^^^^^^^^^^^^
  \if@filesw
    \begingroup
      \let\protect\noexpand
      \immediate\write\@auxout{%
        \string\bibcite{#1}{\the\value{\@listctr}}%
      }%
    \endgroup
  \fi
  \ignorespaces
}%

\def\@citex[#1]#2{%
  \let\@citea\@empty
  \@cite{%
    \@for\@citeb:=#2\do{%
      \@citea
      \def\@citea{,\penalty\@m\ }%
      \edef\@citeb{\expandafter\@firstofone\@citeb}%
      \if@filesw
        \immediate\write\@auxout{\string\citation{\@citeb}}%
      \fi
      \@ifundefined{b@\@citeb}{%
        \mbox{\reset@font\bfseries ?}%
        \G@refundefinedtrue
        \@latex@warning{%
          Citation `\@citeb' on page \thepage \space undefined%
        }%
      }{%
	\hyper@natlinkstart{\@citeb}% \hyper@natlinkstart{#2}%
%       ^^^^^^^^^^^^^^^^^^^^^^^^
            \hbox{\csname b@\@citeb\endcsname}%
        \hyper@natlinkend%
%       ^^^^^^^^^^^^^^^^^^
      }%
    }%
  }{#1}%
}%

\makeatother


==> short_ext.tex <==
% -*- coding:utf-8 -*-

\section{Extension to $\MSO_{2}$}
\label{sec:short-ext}

The $\MSO_{2}$ (or $\GSO$) logic on graphs is a generalization of $\MSO_{1}$ that additionally allows edge variables, edge-set variables,
and an atomic formula $I(x,y)$ meaning that the edge assigned to $y$ is incident to the vertex assigned to  $x$.
Although $\MSO_{2}$ is strictly stronger than $\MSO_{1}$ in general,
for graphs of bounded treewidth,
the model checking problem for $\MSO_{2}$ can be reduced to the one for $\MSO_{1}$ in polynomial time~\cite{CourcelleE12}.
Using a similar reduction, 
we show that the same holds for $\MSOGLLin$ on graphs of bounded vertex integrity.

Now we define the extension of $\MSOGLLin$ with $\MSO_{2}$, which we call $\GSOGLLin$.
In $\GSOGLLin$, 
the local cardinality constraints for vertex-set variables
and the global cardinality constraints work in the same way as in $\MSOGLLin$.
The local cardinality constraints for an edge-set variable $X$ at a vertex $v$
restricts the number of edges in $X$ incident to $v$.
%
A \emph{$\GSOGLLin$ formula} on a $p$-colored graph $\mathcal{G} = (G, \cfun)$ is a tuple $(\varphi, \vect{R}, \vect{\alpha}^G)$,
where $\vect{R} = (R_1, \ldots, R_g)$ and $\vect{\alpha}^G = (\alpha_1^G, \ldots, \alpha_s^G)$ are the global and local cardinality constraints,
and $\varphi$ is an $\MSO_{2}$ formula with $s$ free set variables that 
additionally equipped with symbols $R_{1}, \dots, R_{g}$.
The problem \pname{$\GSOGLLin$ Model Checking} is formalized as follows.
\begin{myproblem}
  \problemtitle{\pname{$\GSOGLLin$ Model Checking}}
  \probleminput{A $p$-colored graph $\mathcal{G} = (G, \cfun)$, and a $\GSOGLLin$ formula $(\varphi, \vect{R}, \vect{\alpha}^G)$.}
  \problemquestiontitle{Question}
  \problemquestion{Is there an assignment $\vect{X}^G = (X_1^G, \ldots, X_s^G)$ of $\varphi$ such that 
  $(\mathcal{G}, \vect{R}, \vect{X}^G) \models \varphi$ and $\vect{X}^G$ obeys $\vect{\alpha}^G$?}
\end{myproblem}

We can show the following theorem by presenting a reduction from from \pname{$\GSOGLLin$ Model Checking} to \pname{$\MSOGLLin$ Model Checking}
(see \cref{sec:ext} for the proof).
\begin{theorem}
\label{thm:gsogl-alg}
\pname{$\GSOGLLin$ Model Checking} is fixed-parameter tractable parameterized by 
$\vi(G)$ and $|\varphi|$.
\end{theorem}
%%
%By Theorem~\ref{thm:msogl-alg}, it suffices to present a polynomial-time reduction 
%from \pname{$\GSOGLLin$ Model Checking} to \pname{$\MSOGLLin$ Model Checking}
%that does not increase the vertex integrity too much.
%Given an instance of \pname{$\GSOGLLin$ Model Checking} that consists of
%a $p$-colored graph $\mathcal{G} = (G=(V,E), \cfun)$ and a $\GSOGLLin$ formula $(\varphi, \vect{R}, \vect{\alpha}^G)$,
%we construct an equivalent instance of \pname{$\MSOGLLin$ Model Checking}.
%Since most of the reduction below is rather standard,
%we basically give the construction only, and add some remarks for important points.
%
%\paragraph*{Modifying the graph.}
%We construct a $(p+1)$-colored graph $\mathcal{G}' = (G', \cfun')$ from $\mathcal{G}$
%by adding a new color consists of new vertices $v_{e}$ for all $e \in E$,
%and adding the edges between $v_{e}$ and the endpoints of $e$ for each $e \in E$.
%That is, 
%$\cfun' = \cfun \tupplus (C_{E})$ with $C_{E} = \{v_{e} \mid e \in E\}$,
%$V(G') = V \cup C_{E}$, and 
%$E(G') = E \cup \{\{u,v_{e}\}, \{w,v_{e}\} \mid e = \{u,w\} \in E\}$.
%%
%Note that we do not forget the original edge set $E$ (which is redundant)
%because handling local cardinality constraints for vertex-set variables is simpler with $E$.
%We can easily see that $\vi(G') \le (\vi(G))^{2}$.
%\begin{observation}
%\label{obs:subdiv}
%If $\vi(G) = k$, then $\vi(G') \le k^{2}$.
%\end{observation}
%\begin{proof}
%Let $S$ be a $\vi(k)$-set of $G = (V,E)$. We show that $S$ is a $\vi(k^{2})$-set of $G'$.
%%
%For $e \in E(G[S])$, the vertex $v_{e}$ forms a singleton component in $G'-S$.
%%
%Let $D$ be a component of $G'-S$ that contains at least one vertex in $V$.
%By the definition of $G'$, 
%there exists a component $C$ of $G-S$ such that
%\[
%  V(D) 
%  = 
%  V(C) 
%  \cup \{v_{e} \mid e \in E(G[C])\} 
%  \cup \{v_{\{u,w\}} \mid \{u,w\} \in E, u \in V(C), w \in S\}.
%\]
%This implies that 
%$|S \cup V(D)| \le |S \cup V(C)| + \binom{|V(C)|}{2}+ |S| \cdot |V(C)| \le k^{2}$.
%\end{proof}
%
%
%\paragraph*{Modifying the formula.}
%From $\varphi$, we obtain a formula $\varphi'$ as follows.
%All edge variables and edge-set variables in $\varphi$ are interpreted
%as vertex variables and vertex-set variables, respectively, with the same names in $\varphi'$.
%The formula $\varphi'$ asks that all ex-edge variables and ex-edge-set variables are taken from $C_{E}$,
%and none of the other variables intersect $C_{E}$. 
%For example, if $Y$ is an edge-set variable in $\varphi$, 
%we replace the maximal subformula $\psi_{Y}$ of $\varphi$ where $Y$ is defined in with 
%$\psi_{Y} \land (\forall y.(\lnot(y \in Y) \lor y \in C_{E}))$, which means $\psi_{Y} \land (Y \subseteq C_{E})$.
%Finally, we replace each $I(x,y)$ in $\varphi$ with $E(x,y)$.
%
%
%
%\paragraph*{Modifying the cardinality constraints.}
%We keep the original local and global cardinality constraints.
%Clearly, the global cardinality constraints work as before since nothing changed for them.
%Observe that the new vertices in $C_{E}$ do not have local cardinality constraints.
%For them, we add dummy local constraints that restrict nothing (e.g., $[0,|V|]$).
%%
%Let $X$ be a set variable in $\varphi'$.
%Recall that $\varphi'$ ensures that $X \subseteq C_{E}$ if $X$ is an edge-set variable in $\varphi$, 
%and $X \cap C_{E} = \emptyset$ otherwise.
%Recall also that $G'$ keeps the original edges in $E$.
%Therefore, the local cardinality constraints for both ex-edge-set variables and ex-vertex-set variables work correctly.

